Solver-Aided Constant-Time Circuit Verification

We present Xenon, a solver-aided method for formally verifying that Verilog hardware executes in constant-time. Xenon scales to realistic hardware designs by drastically reducing the effort needed to localize the root cause of verification failures via a new notion of constant-time counterexamples, which Xenon uses to automatically synthesize a minimal set of secrecy assumptions. Xenon further exploits modularity in Verilog code via a notion of module summaries, thereby avoiding duplicate work across multiple module instantiations. We show how Xenon's assumption synthesis and summaries enable the verification of a variety of circuits including AES, a highly modular AES-256 implementation where modularity cuts verification from six hours to under three seconds, and ScarV, a timing channel hardened RISC-V micro-controller whose size exceeds previously verified designs by an order of magnitude.

==> graph/intro01-non-ct.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u3)  [draw,ellipse] {ex\_in \#7};
  \node (u4) [draw,ellipse, below=of u3] {ex\_out \#10};
  \draw [->,solid] (u3) edge [loop right] (u3);
  \draw [->,solid] (u3) edge (u4);
%
\end{tikzpicture}


==> graph/intro01-non-pub.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (55.895bp,18.0bp) [draw,ellipse] {bubble\#0};
%
\end{tikzpicture}


==> graph/intro02-non-ct.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u2) [draw,ellipse] {p_ex_out \#7};
  \node (u4) [draw,ellipse,below=of u2] {p_out \#8};
  \draw [->,solid] (u2) edge (u4);
%
\end{tikzpicture}


==> graph/intro02-non-pub.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (55.895bp,18.0bp) [draw,ellipse] {bubble\#0};
%
\end{tikzpicture}


==> graph/intro03-non-ct-full.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,scale=0.45]
%%
\definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \node (u0) at (165.1bp,234.0bp) [draw=strokecolor,ellipse] {bubble};
  \node (u9) at (165.1bp,162.0bp) [draw,ellipse] {r3 \#7};
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \node (u2) at (446.1bp,162.0bp) [draw=strokecolor,ellipse] {cond};
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \node (u3) at (446.1bp,90.0bp) [draw=strokecolor,ellipse] {cond\_r};
  \definecolor{strokecolor}{rgb}{0.0,0.35,0.71};
  \node (u8) at (269.1bp,18.0bp) [draw=strokecolor,ellipse] {r2 \#13};
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \node (u4) at (299.1bp,162.0bp) [draw=strokecolor,ellipse] {in};
  \definecolor{strokecolor}{rgb}{0.0,0.35,0.71};
  \node (u6) at (206.1bp,90.0bp) [draw=strokecolor,ellipse] {r1\_1 \#10};
  \definecolor{strokecolor}{rgb}{0.0,0.35,0.71};
  \node (u7) at (332.1bp,90.0bp) [draw=strokecolor,ellipse] {r1\_2 \#10};
  \node (u5) at (48.096bp,90.0bp) [draw,ellipse] {out \#10};
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,dashed] (u0) ..controls (165.1bp,207.98bp) and (165.1bp,198.71bp)  .. (u9);
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,solid] (u2) ..controls (446.1bp,135.98bp) and (446.1bp,126.71bp)  .. (u3);
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,dashed] (u3) ..controls (387.04bp,65.644bp) and (341.71bp,47.717bp)  .. (u8);
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,solid] (u4) ..controls (268.55bp,138.01bp) and (250.42bp,124.36bp)  .. (u6);
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,solid] (u4) ..controls (310.76bp,136.25bp) and (315.49bp,126.22bp)  .. (u7);
  \draw [->,solid] (u6) ..controls (228.95bp,63.606bp) and (238.83bp,52.628bp)  .. (u8);
  \draw [->,solid] (u7) ..controls (309.24bp,63.606bp) and (299.36bp,52.628bp)  .. (u8);
  \definecolor{strokecolor}{rgb}{0.86,0.2,0.13};
  \draw [strokecolor,->,solid] (u8) ..controls (198.99bp,30.507bp) and (161.87bp,43.732bp)  .. (143.1bp,72.0bp) .. controls (130.44bp,91.054bp) and (138.93bp,116.76bp)  .. (u9);
  \draw [->,solid] (u9) ..controls (125.15bp,137.1bp) and (100.84bp,122.55bp)  .. (u5);
  \draw [->,solid] (u9) ..controls (179.64bp,136.16bp) and (185.59bp,126.01bp)  .. (u6);
  \draw [->,solid] (u9) ..controls (219.26bp,138.3bp) and (259.83bp,121.29bp)  .. (u7);
  \draw [->,solid] (u9) ..controls (206.83bp,177.31bp) and (220.79bp,173.04bp)  .. (220.79bp,162.0bp) .. controls (220.79bp,153.55bp) and (212.61bp,149.06bp)  .. (u9);
%
\end{tikzpicture}


==> graph/intro03-non-ct.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u5) [draw,ellipse] {out \#10};
  \node (u9) [draw,ellipse,above=of u5] {r3 \#7};
  \draw [->,solid] (u9) edge (u5);
  \draw [->,solid] (u9) edge [loop right] (u9);
%
\end{tikzpicture}


==> graph/intro03-non-pub.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (55.895bp,18.0bp) [draw,ellipse] {bubble\#0};
%
\end{tikzpicture}


==> graph/stall-non-ct-step-1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (104.48bp,450.0bp) [draw,ellipse] {EX\_MemRead \#7};
  \node (u28) at (314.48bp,378.0bp) [draw,ellipse] {Stall \#10};
  \node (u1) at (469.48bp,90.0bp) [draw,ellipse] {EX\_rt \#7};
  \node (u5) at (113.48bp,306.0bp) [draw,ellipse] {ID\_Jump \#7};
  \node (u13) at (299.48bp,234.0bp) [draw,ellipse] {ID\_instr \#7};
  \node (u6) at (106.48bp,90.0bp) [draw,ellipse] {ID\_Jump\_v \#7};
  \node (u7) at (299.48bp,18.0bp) [draw,ellipse] {ID\_MemRead \#7};
  \node (u8) at (299.48bp,90.0bp) [draw,ellipse] {ID\_MemRead\_v \#7};
  \node (u15) at (299.48bp,162.0bp) [draw,ellipse] {ID\_op \#7};
  \node (u17) at (175.48bp,162.0bp) [draw,ellipse] {ID\_rs \#7};
  \node (u18) at (422.48bp,162.0bp) [draw,ellipse] {ID\_rt \#7};
  \draw [->,dashed] (u0) ..controls (183.74bp,422.58bp) and (232.41bp,406.36bp)  .. (u28);
  \draw [->,dashed] (u1) ..controls (483.06bp,126.37bp) and (490.53bp,155.85bp)  .. (482.48bp,180.0bp) .. controls (457.01bp,256.4bp) and (384.91bp,322.35bp)  .. (u28);
  \draw [->,dashed] (u5) ..controls (180.17bp,279.9bp) and (221.55bp,264.33bp)  .. (u13);
  \draw [->,solid] (u6) ..controls (108.26bp,145.32bp) and (111.12bp,232.98bp)  .. (u5);
  \draw [->,solid] (u7) ..controls (145.18bp,31.515bp) and (48.741bp,45.329bp)  .. (21.478bp,72.0bp) .. controls (-7.4342bp,100.28bp) and (2.4781bp,120.55bp)  .. (2.4781bp,161.0bp) .. controls (2.4781bp,307.0bp) and (2.4781bp,307.0bp)  .. (2.4781bp,307.0bp) .. controls (2.4781bp,356.6bp) and (44.032bp,400.73bp)  .. (u0);
  \draw [->,solid] (u8) ..controls (299.48bp,63.983bp) and (299.48bp,54.712bp)  .. (u7);
  \draw [->,solid] (u13) ..controls (363.97bp,248.68bp) and (381.82bp,244.27bp)  .. (381.82bp,234.0bp) .. controls (381.82bp,225.5bp) and (369.58bp,221.01bp)  .. (u13);
  \draw [->,solid] (u13) ..controls (299.48bp,207.98bp) and (299.48bp,198.71bp)  .. (u15);
  \draw [->,solid] (u13) ..controls (254.17bp,207.42bp) and (230.23bp,193.91bp)  .. (u17);
  \draw [->,solid] (u13) ..controls (344.54bp,207.35bp) and (368.49bp,193.73bp)  .. (u18);
  \draw [->,dashed] (u15) ..controls (233.77bp,137.17bp) and (189.8bp,121.22bp)  .. (u6);
  \draw [->,dashed] (u15) ..controls (299.48bp,135.98bp) and (299.48bp,126.71bp)  .. (u8);
  \draw [->,dashed] (u17) ..controls (194.48bp,198.13bp) and (210.89bp,227.51bp)  .. (226.48bp,252.0bp) .. controls (249.17bp,287.65bp) and (277.68bp,327.31bp)  .. (u28);
  \draw [->,solid] (u18) ..controls (439.21bp,136.08bp) and (446.11bp,125.8bp)  .. (u1);
  \draw [->,dashed] (u18) ..controls (411.83bp,198.37bp) and (402.02bp,227.85bp)  .. (390.48bp,252.0bp) .. controls (373.22bp,288.13bp) and (348.4bp,327.16bp)  .. (u28);
%
\end{tikzpicture}


==> graph/stall-non-ct-step-2.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (457.04bp,882.0bp) [draw,ellipse] {EX\_MemRead \#13};
  \node (u28) at (863.04bp,810.0bp) [draw,ellipse] {Stall \#13};
  \node (u1) at (982.04bp,522.0bp) [draw,ellipse] {EX\_rt \#13};
  \node (u5) at (713.04bp,738.0bp) [draw,ellipse] {ID\_Jump \#10};
  \node (u13) at (658.04bp,666.0bp) [draw,ellipse] {ID\_instr \#10};
  \node (u23) at (825.04bp,522.0bp) [draw,ellipse] {IF\_pc\_jump \#10};
  \node (u6) at (193.04bp,522.0bp) [draw,ellipse] {ID\_Jump\_v \#10};
  \node (u7) at (89.042bp,450.0bp) [draw,ellipse] {ID\_MemRead \#10};
  \node (u8) at (386.04bp,522.0bp) [draw,ellipse] {ID\_MemRead\_v \#10};
  \node (u14) at (608.04bp,594.0bp) [draw,ellipse] {ID\_jaddr \#10};
  \node (u15) at (386.04bp,594.0bp) [draw,ellipse] {ID\_op \#10};
  \node (u17) at (745.04bp,594.0bp) [draw,ellipse] {ID\_rs \#10};
  \node (u18) at (904.04bp,594.0bp) [draw,ellipse] {ID\_rt \#10};
  \node (u16) at (868.04bp,234.0bp) [draw,ellipse] {ID\_pc4 \#10};
  \node (u19) at (203.04bp,90.0bp) [draw,ellipse] {IF\_instr \#10};
  \node (u20) at (109.04bp,18.0bp) [draw,ellipse] {IF\_instr\_tmp \#10};
  \node (u21) at (857.04bp,378.0bp) [draw,ellipse] {IF\_pc \#7};
  \node (u22) at (868.04bp,306.0bp) [draw,ellipse] {IF\_pc4 \#7};
  \node (u24) at (1069.0bp,234.0bp) [draw,ellipse] {IF\_pc\_maybestalled \#7};
  \node (u31) at (544.04bp,306.0bp) [draw,ellipse] {M\_rom32\_V\_address\_T13 \#0};
  \node (u25) at (846.04bp,450.0bp) [draw,ellipse] {IF\_pc\_next \#7};
  \node (u100) at (846.04bp,450.0bp) [draw,ellipse,right=of u25] {M_PCSrc};
  \draw [->,dashed] (u100) -- (u25);
  % \node (u32) at (608.04bp,234.0bp) [draw,ellipse] {M\_rom32\_V\_address\_select\_T13 \#0};
  % \node (u34) at (252.04bp,234.0bp) [draw,ellipse] {M\_rom32\_V\_mem\_offset\_T13 \#0};
  \node (u33) at (252.04bp,162.0bp) [draw,ellipse] {M\_rom32\_V\_data\_out\_T13 \#0};
  \draw [->,dashed] (u0) ..controls (604.67bp,855.55bp) and (732.19bp,833.56bp)  .. (u28);
  \draw [->,dashed] (u1) ..controls (977.27bp,558.22bp) and (972.2bp,587.63bp)  .. (964.04bp,612.0bp) .. controls (942.27bp,677.01bp) and (901.8bp,747.07bp)  .. (u28);
  \draw [->,dashed] (u5) ..controls (693.04bp,711.54bp) and (684.81bp,701.07bp)  .. (u13);
  \draw [->,dashed] (u5) ..controls (750.55bp,697.84bp) and (787.03bp,655.35bp)  .. (806.04bp,612.0bp) .. controls (814.7bp,592.26bp) and (819.53bp,568.27bp)  .. (u23);
  \draw [->,solid] (u6) ..controls (237.66bp,559.02bp) and (281.28bp,591.56bp)  .. (323.04bp,612.0bp) .. controls (434.27bp,666.45bp) and (574.69bp,704.67bp)  .. (u5);
  \draw [->,solid] (u7) ..controls (70.249bp,494.38bp) and (51.042bp,546.55bp)  .. (51.042bp,593.0bp) .. controls (51.042bp,739.0bp) and (51.042bp,739.0bp)  .. (51.042bp,739.0bp) .. controls (51.042bp,806.39bp) and (252.86bp,849.34bp)  .. (u0);
  \draw [->,solid] (u8) ..controls (278.27bp,495.6bp) and (206.51bp,478.69bp)  .. (u7);
  \draw [->,solid] (u13) ..controls (727.37bp,680.62bp) and (746.24bp,676.2bp)  .. (746.24bp,666.0bp) .. controls (746.24bp,657.48bp) and (733.05bp,652.99bp)  .. (u13);
  \draw [->,solid] (u13) ..controls (639.92bp,639.63bp) and (632.53bp,629.28bp)  .. (u14);
  \draw [->,solid] (u13) ..controls (561.89bp,640.25bp) and (487.07bp,621.0bp)  .. (u15);
  \draw [->,solid] (u13) ..controls (690.28bp,639.06bp) and (704.95bp,627.25bp)  .. (u17);
  \draw [->,solid] (u13) ..controls (746.49bp,639.83bp) and (811.72bp,621.27bp)  .. (u18);
  \draw [->,solid] (u14) ..controls (683.74bp,568.58bp) and (733.55bp,552.51bp)  .. (u23);
  \draw [->,dashed] (u15) ..controls (320.33bp,569.17bp) and (276.37bp,553.22bp)  .. (u6);
  \draw [->,dashed] (u15) ..controls (386.04bp,567.98bp) and (386.04bp,558.71bp)  .. (u8);
  \draw [->,solid] (u16) ..controls (788.41bp,270.3bp) and (717.04bp,313.66bp)  .. (717.04bp,377.0bp) .. controls (717.04bp,451.0bp) and (717.04bp,451.0bp)  .. (717.04bp,451.0bp) .. controls (717.04bp,501.92bp) and (672.39bp,545.83bp)  .. (u14);
  \draw [->,dashed] (u17) ..controls (775.03bp,649.39bp) and (824.38bp,738.89bp)  .. (u28);
  \draw [->,solid] (u18) ..controls (931.97bp,567.94bp) and (945.01bp,556.23bp)  .. (u1);
  \draw [->,dashed] (u18) ..controls (897.57bp,641.5bp) and (888.26bp,703.91bp)  .. (877.04bp,756.0bp) .. controls (875.21bp,764.5bp) and (872.9bp,773.69bp)  .. (u28);
  \draw [->,solid] (u19) ..controls (168.84bp,63.533bp) and (153.13bp,51.83bp)  .. (u20);
  \draw [->,solid] (u20) ..controls (81.884bp,76.659bp) and (41.819bp,180.25bp)  .. (82.042bp,252.0bp) .. controls (187.0bp,439.24bp) and (359.06bp,337.11bp)  .. (494.04bp,504.0bp) .. controls (526.04bp,543.56bp) and (497.15bp,574.96bp)  .. (532.04bp,612.0bp) .. controls (549.27bp,630.29bp) and (573.8bp,642.52bp)  .. (u13);
  \draw [->,solid] (u21) ..controls (860.97bp,351.98bp) and (862.43bp,342.71bp)  .. (u22);
  \draw [->,solid] (u21) ..controls (917.2bp,336.7bp) and (992.21bp,286.46bp)  .. (u24);
  \draw [->,solid] (u21) ..controls (764.95bp,356.4bp) and (682.09bp,337.87bp)  .. (u31);
  \draw [->,solid] (u22) ..controls (868.04bp,279.98bp) and (868.04bp,270.71bp)  .. (u16);
  \draw [->,solid] (u22) ..controls (935.99bp,281.34bp) and (979.75bp,266.1bp)  .. (u24);
  % \draw [->,solid] (u23) ..controls (832.57bp,495.9bp) and (835.39bp,486.51bp)  .. (u25);
  % \draw [->,solid] (u24) ..controls (1047.3bp,294.08bp) and (1001.9bp,402.94bp)  .. (932.04bp,468.0bp) .. controls (916.27bp,482.68bp) and (895.67bp,494.18bp)  .. (u23);
  \draw [->,solid] (u25) ..controls (849.97bp,423.98bp) and (851.43bp,414.71bp)  .. (u21);
  % \draw [->,dashed] (u28) ..controls (810.07bp,784.28bp) and (778.93bp,769.75bp)  .. (u5);
  % \draw [->,dashed] (u28) ..controls (636.24bp,790.8bp) and (89.042bp,740.52bp)  .. (89.042bp,667.0bp) .. controls (89.042bp,667.0bp) and (89.042bp,667.0bp)  .. (89.042bp,593.0bp) .. controls (89.042bp,553.0bp) and (89.042bp,506.65bp)  .. (u7);
  % \draw [->,dashed] (u28) ..controls (967.76bp,783.41bp) and (1069.0bp,744.97bp)  .. (1069.0bp,667.0bp) .. controls (1069.0bp,667.0bp) and (1069.0bp,667.0bp)  .. (1069.0bp,377.0bp) .. controls (1069.0bp,337.0bp) and (1069.0bp,290.65bp)  .. (u24);
  % \draw [->,solid] (u31) ..controls (567.28bp,279.58bp) and (576.8bp,269.17bp)  .. (u32);
  % \draw [->,solid] (u31) ..controls (435.12bp,278.89bp) and (374.31bp,264.31bp)  .. (u34);
  % \draw [->,dashed] (u32) ..controls (473.3bp,206.51bp) and (395.84bp,191.27bp)  .. (u33);
  \draw [->,dashed] (u31) -- (u33);
  \draw [->,solid] (u33) -- (u19);
  % \draw [->,solid] (u33) ..controls (392.65bp,175.91bp) and (424.08bp,171.42bp)  .. (424.08bp,162.0bp) .. controls (424.08bp,153.42bp) and (398.05bp,148.93bp)  .. (u33);
  % \draw [->,dashed] (u34) ..controls (252.04bp,207.98bp) and (252.04bp,198.71bp)  .. (u33);
%
\end{tikzpicture}


==> graph/stall-non-pub-step-1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (u0) at (289.39bp,450.0bp) [draw,ellipse] {EX\_MemRead (4)};
  \node (u28) at (289.39bp,378.0bp) [draw,ellipse] {Stall (7)};
  \node (u1) at (557.39bp,90.0bp) [draw,ellipse] {EX\_rt (4)};
  \node (u5) at (289.39bp,306.0bp) [draw,ellipse] {ID\_Jump (4)};
  \node (u13) at (358.39bp,234.0bp) [draw,ellipse] {ID\_instr (4)};
  \node (u6) at (191.39bp,90.0bp) [draw,ellipse] {ID\_Jump\_v (4)};
  \node (u7) at (88.392bp,18.0bp) [draw,ellipse] {ID\_MemRead (4)};
  \node (u8) at (383.39bp,90.0bp) [draw,ellipse] {ID\_MemRead\_v (4)};
  \node (u15) at (358.39bp,162.0bp) [draw,ellipse] {ID\_op (4)};
  \node (u17) at (237.39bp,162.0bp) [draw,ellipse] {ID\_rs (4)};
  \node (u18) at (479.39bp,162.0bp) [draw,ellipse] {ID\_rt (4)};
  \node (u30) at (576.39bp,522.0bp) [draw,ellipse] {reset (0)};
  \draw [->,dashed] (u0) ..controls (289.39bp,423.98bp) and (289.39bp,414.71bp)  .. (u28);
  \draw [->,dashed] (u1) ..controls (554.53bp,126.82bp) and (550.0bp,156.84bp)  .. (538.39bp,180.0bp) .. controls (500.29bp,256.03bp) and (481.14bp,273.94bp)  .. (412.39bp,324.0bp) .. controls (389.18bp,340.9bp) and (359.74bp,353.83bp)  .. (u28);
  \draw [->,dashed] (u5) ..controls (314.51bp,279.52bp) and (325.46bp,268.41bp)  .. (u13);
  \draw [->,solid] (u6) ..controls (176.55bp,126.25bp) and (168.23bp,156.04bp)  .. (177.39bp,180.0bp) .. controls (193.71bp,222.67bp) and (232.05bp,259.96bp)  .. (u5);
  \draw [->,solid] (u7) ..controls (69.599bp,62.377bp) and (50.392bp,114.55bp)  .. (50.392bp,161.0bp) .. controls (50.392bp,307.0bp) and (50.392bp,307.0bp)  .. (50.392bp,307.0bp) .. controls (50.392bp,383.02bp) and (140.86bp,419.25bp)  .. (u0);
  \draw [->,solid] (u8) ..controls (276.45bp,63.625bp) and (205.37bp,46.757bp)  .. (u7);
  \draw [->,solid] (u13) ..controls (422.37bp,248.68bp) and (440.09bp,244.27bp)  .. (440.09bp,234.0bp) .. controls (440.09bp,225.5bp) and (427.94bp,221.01bp)  .. (u13);
  \draw [->,solid] (u13) ..controls (358.39bp,207.98bp) and (358.39bp,198.71bp)  .. (u15);
  \draw [->,solid] (u13) ..controls (314.18bp,207.42bp) and (290.82bp,193.91bp)  .. (u17);
  \draw [->,solid] (u13) ..controls (402.72bp,207.35bp) and (426.28bp,193.73bp)  .. (u18);
  \draw [->,dashed] (u15) ..controls (300.65bp,136.8bp) and (264.64bp,121.7bp)  .. (u6);
  \draw [->,dashed] (u15) ..controls (367.26bp,136.18bp) and (370.67bp,126.62bp)  .. (u8);
  \draw [->,dashed] (u17) ..controls (214.34bp,210.75bp) and (189.72bp,276.36bp)  .. (214.39bp,324.0bp) .. controls (222.03bp,338.75bp) and (235.87bp,350.27bp)  .. (u28);
  \draw [->,solid] (u18) ..controls (507.39bp,135.87bp) and (520.55bp,124.07bp)  .. (u1);
  \draw [->,dashed] (u18) ..controls (472.6bp,199.2bp) and (464.51bp,229.74bp)  .. (449.39bp,252.0bp) .. controls (417.26bp,299.31bp) and (361.59bp,336.86bp)  .. (u28);
  \draw [->,dashed] (u30) ..controls (488.96bp,499.67bp) and (409.98bp,480.41bp)  .. (u0);
  \draw [->,dashed] (u30) ..controls (595.19bp,477.62bp) and (614.39bp,425.45bp)  .. (614.39bp,379.0bp) .. controls (614.39bp,379.0bp) and (614.39bp,379.0bp)  .. (614.39bp,233.0bp) .. controls (614.39bp,189.56bp) and (591.14bp,143.68bp)  .. (u1);
  \draw [->,dashed] (u30) ..controls (527.08bp,456.31bp) and (420.77bp,316.83bp)  .. (u13);
%
\end{tikzpicture}


==> modules.tex <==
\section{Modules}

==> prelims.tex <==
\section{Preliminaries}
